Perceptual Grouping in Contrastive Vision-Language Models

Recent advances in zero-shot image recognition suggest that vision-language models learn generic visual representations with a high degree of semantic information that may be arbitrarily probed with natural language phrases. Understanding an image, however, is not just about understanding what content resides within an image, but importantly, where that content resides. In this work we examine how well vision-language models are able to understand where objects reside within an image and group together visually related parts of the imagery. We demonstrate how contemporary vision and language representation learning models based on contrastive losses and large web-based data capture limited object localization information. We propose a minimal set of modifications that results in models that uniquely learn both semantic and spatial information. We measure this performance in terms of zero-shot image recognition, unsupervised bottom-up and top-down semantic segmentations, as well as robustness analyses. We find that the resulting model achieves state-of-the-art results in terms of unsupervised segmentation, and demonstrate that the learned representations are uniquely robust to spurious correlations in datasets designed to probe the causal behavior of vision models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/experiments_old.tex <==
%\vspace{-0.5cm}
\section{Experiments}
%\subsection{Experimental Setup}
\label{section:experiment-overview}

\input{sections/latex-figures/table-image-recognition}
\input{sections/latex-figures/figure-jaccard-refactor}
\input{sections/latex-figures/jaccard-cityscapes}

{\bf Experimental Setup.} We train vision-language models on two datasets: Conceptual Captions 12M (CC-12M) \citep{changpinyo2021conceptual} and High Quality Image Text Pairs (\datasetname-134M) consisting of 12 million and 134 million image-text pairs, respectively (App. \ref{section:internal-dataset} for details).
For both datasets, text is  tokenized, and images resized and center cropped to 224$\times$224 pixels. We report results on EfficientNet-B5 employed by ALIGN \cite{jia2021scaling}, and ViT-B/16 employed by CLIP \cite{radford2021clip} although we focus more on the latter.
We train models on 32 GPUs across 4 machines with PyTorch \cite{NEURIPS2019_bdbca288}. See App. \ref{section:training-details} for details.


We evaluate the model across image classification, localization, and robustness tasks. Results are based on zero-shot analyses where the model is prompted at inference for a selection of labels (App. \ref{section:prompts} for prompts). For image classification, we employ the validation splits of ImageNet \citep{deng2009imagenet}, ImageNet-v2 \citep{recht2019imagenet}, and the test split of Waterbirds \cite{sagawa2019distributionally}.

For segmentation tasks, we employ zero shot analysis at each spatial location. This is performed by employing the CAM method \cite{ghiasi2021simple,zhou2016learning} to generate a prediction across space by exploiting the transitive property of average pooling and argmax. To measure success, we employ the validation splits of PASCAL VOC \citep{everingham2010pascal}, ADE20K \citep{zhou2018ade,cheng2021maskformer} and COCO \citep{coco}. Each dataset contains 20, 150 and 133 labels, respectively.

Given that most competitive baselines are trained on private datasets, we first attempt to reproduce results by designing and training vision-language models on a corpus of image-text pairs. In more detail, we train on \datasetname-134M, and observe competitive performance given our data limitations. We also train and report results on the public CC-12M dataset to provide reproducible numbers. We measure the performance of CLIP and ALIGN on zero-shot image classification on ImageNet and ImageNet-v2. We evaluate all of the proposed architectural changes in Sec.~\ref{sec:methods}, which in aggregate we term \modelname, and thoroughly analyse them.

Tab. \ref{table:image-recognition} highlights our results on zero-shot image classification. We take this as a starting point for subsequent work.
In the following experiments we attempt to address the following questions:\setlist{nolistsep}
    \begin{itemize}[noitemsep]
    \item What are the limitations of current vision-language models? (Fig. \ref{fig:motivation})
    \item Do we observe perceptual grouping in vision language models? (Fig. \ref{figure:jaccard-similarity}, Tab. \ref{table:semantic-segmentation}).
    \item How resilient are vision-language models to counterfactual manipulations? (Fig. \ref{figure:robustness}).
    \item How important are each of the proposed model modifications? (Tab. \ref{table:ablations}).
\end{itemize}


\input{sections/latex-figures/table-segmentation}

%\vspace{-0.2cm}
\subsection{Limitations of vision-language models}

Visual representations learned in vision-language models exhibit an impressive ability to generalize across tasks \cite{radford2021clip,jia2021scaling}. However these models also exhibit a profound shortcoming -- learned visual representations maintain minimal information about {\it where} an object resides, failing to properly recognize what parts of an image constitute an object.
%the actual object of interest.

Fig. \ref{fig:motivation} (bottom row) showcases failure of a CLIP model; namely, the model improperly conflates visual content not associated with an object with the actual object. This can be observed by measuring the similarity of each embedding at each spatial location with a label set using the CAM method (Sec. \ref{section:experiment-overview}). One consistently observes that the central object of interest is incorrectly predicted to reside at every spatial location. For instance, in the left example, the CLIP model predicts that a {\tt bird} resides at every spatial location.
In a CNN architecture, where spatial information is inherently preserved, we observe some improvement, but the larger issue of poor localization remains (see App. \ref{section:cnn-analysis} for details).

The failure of vision-language models to properly understand the spatial organization of information is consistent with earlier observations.
Ablation experiments in ViT models demonstrated that removing positional embeddings minimally detriments predictive performance \cite{dosovitskiy2020image,naseer2021intriguing,pmlr-v162-zhai22a,subramanian2022reclip}.
Without positional information, ViT models effectively learn representations as a ``bag of image patches'', ignoring the spatial organization.

In contrast, if we perform the same analysis on \modelname, we see that the model retains significant information about spatial information (Fig. \ref{fig:motivation}, bottom right). We take these visualizations as an impetus for further investigation. In particular, we start by quantifying the ability of the model to arbitrarily group together semantically related pixels, and compare this to previous works.

\subsection{Emergence of Bottom-Up Perceptual Grouping}
% \modelname groups semantically related visual inputs

Performance on segmentation unsupervised by true object masks at training time is a direct measure of bottom up perceptual grouping.  We apply \modelname at test time to perform semantic segmentation without prompting it for any labels \footnote{We follow the procedure outlined by \citet{caron2021emerging}. Namely, we compute PCA across the spatial map of image features. Each principal component corresponds to a candidate feature and we cluster the proximity of each feature vector to these components. GroupViT \cite{xu2022groupvit} and DINO \cite{caron2021emerging} employ 8 and 6 feature vectors based on their model architectures. For our visualizations, we employ 8 feature vectors.}. Fig. \ref{figure:jaccard-similarity}b shows that the model visually groups semantically related regions of an image (see also Fig. \ref{fig:qualitative-bottom-up-segmentation-examples}) as the image embeddings naturally group into spatially distinct clusters mirroring the image structure. We emphasize that this analysis does \textit{not} rely on text prompts \textit{nor} segmentation labels, but merely emerges from the image features alone. Hence the model has learned to \textit{group} perceptually related pixels merely based on the pixel content and associated text (see App. \ref{section:prior-unsupervised-segmentation} for more).

We quantify the accuracy of this bottom-up segmentation to capture known segmentations within annotated images. We follow \citet{caron2021emerging, xu2022groupvit} to perform a matching between all candidate annotations with a given segmentation proposed by the model. We compute the Jaccard Similarity (JS) between the inferred segmentations and the associated annotation. The JS measures the average intersection over the union across all segmentation instances regardless of object identity.

On Pascal VOC, Fig. \ref{figure:jaccard-similarity}a shows that \modelname achieves $54.6\%$ outperforming all previous models; in comparison, CLIP achieves 38.9\%. Additionally, we tested the model on two  more challenging datasets and note that the model drops in performance, perhaps indicative of more visually cluttered scenes (Fig. \ref{figure:jaccard-similarity}c).
We take the results to indicate that \modelname perceptually groups semantically related content better than previous work, and provides state-of-the-art results in unsupervised segmentation. 

\subsection{Top-down Object Grouping}

We demonstrated that \modelname is able to perceptually group visual content within an image.
Next, we ask how well this perceptual grouping corresponds to semantically meaningful labels. 
To measure the emergence of top-down processing, we ask how well the perceptual grouping of the model may be steered by embeddings from the language model.
We test this hypothesis by comparing the model's ability to perform zero-shot semantic segmentation across three datasets. Note that all of our results and comparisons are solely restricted to models trained on \textit{no} segmentation annotations \footnote{In App. \ref{section:prior-zemantic-segmentation}, we provide a summary of other zero-shot semantic segmentation results. Some of these prior results achieve superior performance, but we note that all of these results were trained explicitly on various forms of segmentation masks, if not the segmentation labels. These models were tested in terms of zero-shot semantic segmentation through a careful split of training and testing labels.
}.

Fig. \ref{fig:motivation} provides a visualization of the predicted zero-shot segmentations (see also App. \ref{section:appendix-qualitative}), and Tab. \ref{table:semantic-segmentation} quantifies the results using mean intersection over union (mIoU). \modelname outperforms all other approaches on semantic segmentation when trained on the same datasets, both for CC-12M and HQITP-134M.
For example, on HQITP-134M, \modelname achieves 51.0\% while our baseline CLIP achieves 18.1\% IoU.
Correspondingly, the official, trained CLIP implementation achieves 16.4\% mIoU. We also tested an internal implementation of an ALIGN model based on a CNN backbone and achieved improved results, as may be expected given the strong spatial prior imposed by the model, however notably below previous state-of-the-art (App. \ref{section:cnn-analysis} for details).

GroupViT provides an important point of comparison \cite{xu2022groupvit}. This model is a custom ViT architecture trained on vision and text pairs designed to perform perceptual grouping by optimizing a discretized attention mask. GroupViT was trained on a comparable dataset of CC-12M, yet our simple changes outperform this custom architecture by over 10 percentage points (41.1 vs. 50.8). 
\footnote{We note that even removing all pretraining data and solely training on CC-12M still retains notable performance on unsupervised segmentation (%i.e. 43.1 vs 41.1, 
see Tab. \ref{table:ablations}).}. %\todo{KR: wrong footnote number - remove?}
We take these results to mean that our simple changes to existing vision-language models uncover powerful localization information.


\input{sections/latex-figures/figure-robustness}

\subsection{Perceptual grouping may improve robustness}
\label{sec:robustness}
%\subsection{Perceptual grouping may be robust to counterfactual examples}
%\subsection{Robustness to Segmentation-related Data Perturbation}
% \subsection{Robustness to spurious correlations}
% \subsection{Robustness to spurious correlations and counterfactual manipulations}
% \subsection{Perceptual grouping provides a robust visual representation}


We have observed how parsimonious changes to vision-language models result in state-of-the-art unsupervised and zero-shot semantic segmentation. In this section, we ask how the resulting perceptual grouping may be exploited to improve the robustness of image understanding. 
A large literature has consistently observed that models systematically underperform under domain shifts \cite{recht2019imagenet}. For instance, CLIP, ALIGN and \modelname underperform on ImageNet-v2 versus ImageNet validation (Tab. \ref{table:image-recognition}). Another means of assessing robustness is to measure how well a model \textit{causally} predicts the label from the appropriate input variates \cite{pearl2009causality,pearl2018book}. To probe for causal dependencies, one can measure model performance to counterfactual examples where an input is selectively manipulated in order to test for sensitivity to spurious correlations.  

A common formulation for this problem is to artificially synthesize a malicious dataset where a trained model may correlate inappropriate image features to predict a label \cite{xiao2020noise,moayeri2022comprehensive,jacobsen2018excessive,arjovsky2019invariant}. A large class of supervised learning algorithms have been developed to train on these datasets \footnote{Synthetic datasets are deliberately constructed to contain a class imbalance such that a minority class may be particularly prone to systematic worse performance. Consequently, experimenters have focused on the worse-case performance on the minority class \cite{sagawa2019distributionally,liu2021just}. Our work is instead focused on the domain gap to target the degree to which spurious correlations inappropriately influence predictions.}
with the aim of mitigating such spurious correlations \cite{sagawa2019distributionally,liu2021just,nam2020learning}.
One common synthetic benchmark is \textit{Waterbirds} \cite{sagawa2019distributionally} which places segmentations of birds in front of a background of land or water. The goal of any prediction system is a two-way classification of whether or not a bird is from the \texttt{waterbird} or \texttt{landbird} category. What makes this problem particularly challenging is when the background is not commensurate with the type of bird. For instance, a trained model may be prone to predict the type of bird due to the presence of water in the background in lieu of the visual appearance of the actual bird.

 
%A common formulation for this problem is to artificially synthesize a malicious dataset where a trained model may correlate inappropriate image features to predict a label \cite{xiao2020noise,moayeri2022comprehensive,jacobsen2018excessive,arjovsky2019invariant}. Typically in these settings the synthetic dataset contains an imbalance in class labels such that a minority class may be prone to systematically worse performance. Consequently, a large class of supervised learning algorithms have been developed to train on these datasets with the aim of avoiding such spurious correlations and predicting better on the minority label class \cite{sagawa2019distributionally,liu2021just,nam2020learning}.

 
%One of the greatest challenges in image recognition is to build robust image features agnostic to spurious correlations present in a dataset \cite{arjovsky2019invariant,liu2021just,sagawa2019distributionally,jacobsen2018excessive,nam2020learning} (see also \cite{geirhos2021partial,recht2019imagenet}). A common formulation for this problem is to artificially synthesize a malicious dataset where a trained model clues into an inappropriate image features to predict a label \cite{xiao2020noise,moayeri2022comprehensive}. Typically in these settings the synthetic dataset contains an imbalance in class labels such that a minority class may be prone to systematically worse performance. Consequently, a large class of supervised learning algorithms have been developed to train on these toy examples with the aim of avoiding such spurious correlations and predicting better on the minority label class.


We first asked how our baseline CLIP model performs on this task when presented with a zero-shot three-way classification task (App. \ref{section:waterbirds-details} for inference procedure). Model performance depends heavily on the background (Fig. \ref{figure:robustness}b). For instance, the prediction accuracy of \texttt{waterbirds} drops by $\Delta$=32.1\% (80.2 $\rightarrow$ 48.1) in the presence of an incommensurate background. Clearly, the baseline CLIP model performs zero-shot prediction by relying on features from the background.

We next asked how \modelname performs given that it exhibits a unique ability to discriminate the spatial locations of objects. Fig. \ref{figure:robustness}a shows selected examples from each class colored by the prediction at each spatial location. Clearly, the model is able to discriminate which locations correspond to each category. We quantify model accuracy across each task, and find the model far less sensitive to the background. For instance, in the case of waterbirds, \modelname  accuracy, while slightly less than the baseline CLIP model, only drops by $\Delta$ = 2.0\% (76.9 $\rightarrow$ 74.9) in spite of the background change (Fig. \ref{figure:robustness}c). 
Interestingly, the domain gap $\Delta$ is minimal ($\sim$4\%) around a broad range of image input resolutions centered about the training resolution of the model (Fig. \ref{figure:robustness}d).
Hence, \modelname, while still susceptible to some spurious correlations, is far more robust than a standard vision-language model.

%We next ask how in-domain performance predicts out-of-domain performance. To address this question, we measured the domain gap $\Delta$ over a range of input resolutions for \modelname (Figure \ref{figure:robustness}, bottom right). The performance on in-domain categories (e.g. waterbirds on water) remains relatively constant (77-83\%) over a wide range of input resolutions. The domain gap $\Delta$ is minimal around the training resolution of the model ($\sim$4\%), but systematically grows as the input resolution diverges further from the training resolution ($\sim$28\%). We take these results to indicate that out-of-domain performance may be largely independent of in-domain performance.
\input{sections/latex-figures/table-ablations}

As points of comparison, all prior work train a supervised model on the training split. In contrast, our predictions are zero-shot, and we do not use the training set. This difference makes a direct comparison of the raw accuracy difficult. That said, the best supervised training methods achieve a domain gap $\Delta$ of 4\% to 8\% (Tab. 1 and priv. correspondence, \citet{liu2021just}), comparable to our results. We take these results to indicate that our zero-shot approach leveraging perceptual grouping provides another approach for addressing spurious correlations and learning robust image features.

\subsection{Ablations Studies}
\label{section:ablations}

We next performed a set of experiments to demonstrate how individual factors in \modelname led to improved localization performance. We first explored the selection of the aggregation method. Our model employs a maximum operation over all spatial locations. We likewise trained models which performed spatial averaging or employed the class token in ViT. Tab. \ref{table:ablations} (left) shows results across two training sets. We see that standard procedures of class token and average pooling result in similar performance on zero-shot classification on ImageNet, but notable reductions in mIoU on Pascal VOC semantic segmentation. For instance, on the model trained with CC-12M, the mIoU on PASCAL VOC dropped from 50.8\% to 4.0\% representing a relative drop of 91.3\%. Similarly, in the case of bottom-up segmentation on the same dataset, we demonstrate a 10 point drop in JS. 

We also explored how the selection of the pretraining method effected the overall performance. Tab. \ref{table:ablations} (right) explores the selective removal of pretraining on the image model, language model or both. All models employ the maximum pooling aggregation across spatial locations. Again, we see that \modelname exhibits significant drops in both zero-shot image recognition and localization by selectively dropping out each pre-training step. For instance, in the model trained on CC-12M, model performance drops from 42.3\% to 25.6\% top-1 accuracy. Likewise, the semantic segmentation mIoU drops from 50.8\% to 23.5\% accuracy.
For bottom-up segmentation, initializing from pretrained models benefits from scaling up the joint training data (Tab. \ref{table:ablations} vs. \ref{table:ablations-internal-data-init}). We suspect that these results indicate that each initialization provides valuable prior information not readily available in joint training for eliciting strong localization properties.






==> sections/intro_old.tex <==
\section{Introduction}

\input{sections/latex-figures/figure-intro}

Learning a representation for visual imagery requires resolving not only what resides within an image, but also where that information resides \cite{marr1982vision}. In many applications, knowledge of {\it where} information resides is sometimes more important than a precise description of the content \cite{geiger2012we,sun2020scalability}. Hence, our ability to learn more generic and robust visual representations requires learning the geometry of visual semantics, and how visual information may be grounded by specific regions of the visual field.

Vision-language models have demonstrated a remarkable ability to learn generic visual representations that may be readily reused across a large array of visual tasks and domains \cite{jia2021scaling,radford2021clip,yu2022coca,desai2021virtex}. Such models are trained on extremely large corpora of weakly labeled image and text (caption) pairs using contrastive and/or caption based losses, yet the resulting learned representations are quite robust, and may be arbitrarily probed for open-vocabulary (i.e. zero-shot) image recognition problems.

Although vision-language modeling provides a considerable advance towards a generic visual representation \cite{geirhos2021partial},
the learned representations demonstrate a profound inability to associate visual content with individual objects (Fig. \ref{fig:motivation}, bottom row). In other words, models trained on large weakly-supervised data have a limited ability to group together visually related content \cite{ghiasi2022open}. Because the representations have a poor understanding of {\it where} an object resides, they easily conflate background with foreground content.
Hence, the learned representations are unable to learn the spatial layout of a scene \cite{subramanian2022reclip,thrush2022winoground}, and are susceptible to learning spurious correlations between a semantic label and extraneous content \cite{sagawa2019distributionally,liu2021just}.


In this work, we wish to build vision-language models which learn from weakly labeled data, but have the added benefit of properly learning where visual content resides within an image. Previous attempts have considered elaborations of vision-language architectures that leverage additional training data, specalized architectures or heuristics \cite{ghiasi2022open,xu2022groupvit,yao2022filip}. We instead focus on building a system that is able to perceptually group regions of visual imagery by identifying a minimal number of changes to existing vision-language models to encourage spatial localization. We find that three small adjustments -- employing self-supervised pretraining, adjusting feature aggregation across space, and token sub-sampling -- results in models that are equally effective in zero-shot image recognition, but also retain spatial information about object locations (Fig. \ref{fig:motivation}, 3rd row).

The resulting model termed \modelname exhibits \textit{perceptual grouping} -- that is, the ability to select and combine related visual signals into semantically meaningful regions  \cite{wertheimer1923,marr1982vision,roelfsema2006cortical}. Endowing models with perceptual grouping -- whether in a bottom up or top down manner -- in learned representations has been a long standing goal in computer vision \cite{malik2001visual,malik2016three}. In this work, our contributions are as follows:
\setlist{nolistsep}
    \begin{itemize}[noitemsep,leftmargin=*]
\item Identify and characterize the systematic failure of vision-language models to properly identify where objects reside within an image, and group together semantically related content.
\item Design a minimal set of changes to endow a model with perceptual grouping. The resulting model achieves state-of-the-art zero-shot segmentation \textit{without} training on \textit{any} segmentation data.
\item Emergence of localization ability in our models uniquely leads to robustness to counterfactual manipulations. The degree of robustness matches if not surpasses previous state-of-the-art supervised learning methods employing specialized training methodologies.
%\item Demonstrate that the resulting model is uniquely robust to counterfactual manipulations due to its knowledge of where an object resides. The degree of robustness is on par if not surpasses previous state-of-the-art specialized supervised learning methods.
%\item A simple recipe to endow current vision-language models with localization capabilities.
%\item The resulting models exhibit state-of-the-art on segmentation results where no groundtruth regions are used. We observe strong results both on bottom-up segmentation benchmarks, where we ask the model to give us perceptual region groupings, as well as on top-down segmentation benchmarks, where we ask the model to segment objects of user-specified class.
%\item Our models exhibit robustness to malicious image perturbations related to localization. In particular, the models are resilient to classification of objects when intentionally placed on unnatural backgrounds.
%\item The resulting models uniquely exhibit robustness to spurious correlations. Unlike other vision-language or image recognition models, our model learns to only associate visual content with only the object of interest, and avoids making predictions based on spurious correlations with background content.
\end{itemize}

% The model in turn exhibits a state-of-the-art ability to perform unsupervised segmentation. We exploit this perceptual grouping to achieve competitive zero-shot semantic segmentation. More importantly, we demonstrate that the resulting model exhibits increased robustness and generalization across domains, suggesting that the learned representation may be more generic and robust for generic vision tasks. \todo{Revise?} 





==> sections/latex-figures/ablate-pretraining.tex <==
\begin{table}[t]
\captionsetup{font=scriptsize}
\begin{minipage}{\linewidth}
\scriptsize
\def\arraystretch{0.8}%  1 is the default
\centering
\begin{tabular}{c|c|c|c|c}
\toprule
I-P & I-F & T-F & IN & VOC \\ \midrule
Cls & \cmark & \xmark & 39.9 & 3.4 \\
Max & \cmark & \xmark & 24.2 & 10.4 \\
Max & \xmark & \cmark & 35.9 & 29.5 \\
Max & \xmark & \xmark & \textbf{42.3} & \textbf{50.8} \\ \bottomrule
\end{tabular}
\vspace{-1.1em}
\caption{\textbf{Frozen encoder:} I-P refers to pooling in image head. I-F (image-head frozen) and T-F (text-head frozen) reduce performance. Trained on CC-12M.}
\label{tbl:freeze_ablation}
\end{minipage}
\end{table}

==> sections/latex-figures/ablate-subsampling.tex <==
\begin{table}[t]
% \begin{minipage}{0.39\textwidth}
\centering
\scalebox{0.90}{
\def\arraystretch{1.0}
\begin{tabular}{c|cccc}
\toprule
Sub-sampling & IN   & VOC  & COCO & ADE-20K \\ \midrule
\xmark    & 45.3 & 50.9 & 23.5 & 12.6    \\ 
\cmark    & 45.6 & 51.8 & 24.1 & 13.4    \\  \bottomrule
\end{tabular}}
% \end{minipage}
% \hspace{0.01\textwidth}
% \begin{minipage}{0.59\textwidth}
\vspace{-0.5em}
\caption{\small {\bf Ablation on proposed patch sub-sampling.} Models are trained on the CC-12M dataset. We highlight that results in this table are reported for a single run (while our best result in the main paper reports averages across three runs).}
\label{table:ablate-subsample}
% \end{minipage}
\end{table}

==> sections/latex-figures/figure-robustness-old.tex <==
\begin{figure*}[t]%
%\scriptsize
\hspace{0.5em}
\begin{subtable}[valign=t]{0.03\textwidth}
    A. \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ % hack!
\end{subtable}
\begin{subtable}[valign=t]{0.60\textwidth}
%\centering
%\begin{minipage}{0.63\linewidth}
\includegraphics[width=1.0\textwidth]{figures/Waterbird-Examples-4.jpg}
%\end{minipage}\hfill
\end{subtable}
% \hspace{1em}
\begin{subtable}[valign=t]{0.03\textwidth}
    B. \\ \\ \\  % hack!
    C. \\ \\ \\ \\  % hack!
    D. \\ \\ \\ \\ \\ \\ % hack!
\end{subtable}
\hspace{-1em}
\begin{subtable}[valign=t]{0.32\textwidth}
%\begin{minipage}{0.35\linewidth}
\centering
\hspace{0.2cm}
\def\arraystretch{1.3}%  1 is the default, change whatever you need
%\small
\scriptsize
\begin{tabular}{c|cc|c}
    \toprule
   CLIP & water & land & $\Delta$ \\
   \shline
   waterbird & 80.2 & 48.1 & {\bf \textcolor{red}{-32.1}}\\
   landbird & 38.8 & 71.7 & {\bf \textcolor{red}{-32.9}} \\
   \bottomrule
\end{tabular} 
\vspace{0.1cm} \\
\hspace{0.2cm}
\begin{tabular}{c|cc|c}
    \toprule
   \modelname & water & land & $\Delta$ \\
   \shline
   waterbird & 76.9 & 74.9 & {\bf \textcolor{red}{-2.0}} \\
   landbird & 80.0 & 84.1 & {\bf \textcolor{red}{-4.1}}  \\
   \bottomrule
\end{tabular} \\
%\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{figures/Robustness-vs-Resolution-Landbirds.jpg}
%\vspace{0.4cm}
%\end{minipage}
\end{subtable}
\vspace{-1em}
\caption{ \textbf{Perceptual grouping mitigates sensitivity to spurious correlations.} (A) Selected examples of waterbirds and landbirds on each background, respectively. The right panel shows the argmax of similarity between the three prompts and the image embedding at each spatial location for \modelname. (B) Accuracy on the {\it test} split (5794 examples) of Waterbirds on CLIP and (C) \modelname evaluated at 448$\times$448 resolution. The domain gap $\Delta$ reports the drop in accuracy between on and off diagonal entries within a row. (D) Zero shot accuracy of \modelname across image resolution for landbirds on land (top) and water (bottom). Note log axis. Shading highlights $\Delta$.}
\label{figure:robustness}
\vspace{-0.3cm}
\end{figure*}

% Our model 54 at 6K
%water-waterbird:   494 / 642 correct (76.9% +/- 1.66%)
%water-landbird:   1804 / 2255 correct (80.0% +/- 0.84%)
%land-waterbird:   481 / 642 correct (74.9% +/- 1.71%)
%land-landbird:   1896 / 2255 correct (84.1% +/- 0.77%)
%total:   4675 / 5794 correct (80.7% +/- 0.52%)


%# Our baseline CLS model
%water-waterbird:   515 / 642 correct (80.2% +/- 1.57%)
%water-landbird:   874 / 2255 correct (38.8% +/- 1.03%)
%land-waterbird:   309 / 642 correct (48.1% +/- 1.97%)
%land-landbird:   1616 / 2255 correct (71.7% +/- 0.95%)
%total:   3314 / 5794 correct (57.2% +/- 0.65%)



% VALIDATION SPLIT
%\begin{tabular}{c|cc|c}
%   %& \small{DINO} & \small{T5} & & \\
%   \modelname & water & land & delta \\
%   \hline
%   waterbird & 75.9 & 74.4 & {\bf \textcolor{red}{-1.5}} \\
%   landbird & 78.3 & 86.5 & {\bf \textcolor{red}{-8.2}}   \\
%\end{tabular}
%\vspace{0.6cm} \\
%\begin{tabular}{c|cc|c}
%   %& \small{DINO} & \small{T5} & & \\
%   CLIP & water & land & delta \\
%   \hline
%   waterbird & 79.7 & 52.6 & {\bf \textcolor{red}{-27.1}} \\
%   landbird & 41.6 & 69.8 & {\bf \textcolor{red}{-28.2}}   \\
%\end{tabular}

==> sections/latex-figures/table-grounding.tex <==
\begin{table}[tb]%

%\scriptsize
\centering
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\begin{tabular}{@{ }l|cc|ccc}
   & \small{segment} & \small{segment} & & & \\
   & \small{label?} & \small{mask?} & \small{ADE20K} & \small{COCO} & \small{PASCAL VOC} \\
   \hline
   LSeg+ & \cmark & \cmark & 30.8 & \,\,\,\,60.8 $^\dagger$ & \\
   ALIGN w/ proposal & & \cmark & 25.3 & \,\,\,\, 23.6 $^\dagger$ & \\   
   OpenSeg & & \cmark & 41.0 & \,\,\,\, 48.2 $^\dagger$ & \\
   OpenSeg + Narr. & & \cmark & 45.5 & \,\,\,\, 48.2 $^\dagger$ & \\
   \hline
   ALIGN & & & 25.7 & 28.2 & \\      
   GroupViT (CC12M) & & & & &  \\      
   GroupViT (CC12M+YFCC) & & & & &  \\
   \modelname (CC12M) & & & 24.5 & 33.6 & 54.0 \\
\end{tabular}
\caption{ \textbf{\modelname provides better grounding.} All numbers report the grounding mIoU for semantic segmentation on ADE20K (150 labels), PASCAL-VOC (20 labels) and COCO (50 labels). Top rows show models trained on segmentation data. Bottom rows show models not trained on any segmentation data. $\dagger$ indicates models that were trained on image segmentation masks from the COCO dataset.}
\label{table:grounding}  
\end{table}


==> sections/latex-figures/table-image-recognition.tex <==
%\begin{wraptable}[16]{r}{6.3cm}
\begin{table}[t]%
\small
\centering
\def\arraystretch{1.2}%  1 is the default, change whatever you need
%\vspace{-0.5cm}
\begin{tabular}{c|c|cc}
\toprule
  & Dataset & IN & IN-v2 \\
   \shline
   ALIGN \cite{jia2021scaling} &  ALIGN-1800M & 76.4 & 70.1 \\
   CLIP \cite{radford2021clip} &  CLIP-400M & 65.5 & 60.8 \\
   \hline
   CLIP $^\dagger$ &  CC-12M & 46.0 & 40.3 \\
   GroupViT \cite{xu2022groupvit} & CC-12M+YFCC & 42.9 & - \\
   GroupViT $^\dagger$  & CC-12M & 25.6 & 23.8 \\
   \modelname & CC-12M & 45.3 & 40.0 \\
   \hline
   %\;\;ALIGN $^*$ & 135M & Internal & \todo{57.5} & \todo{?} \\
   ALIGN $^\dagger$ &  \datasetname-134M & 51.1 & 45.6 \\
   CLIP $^\dagger$ &  \datasetname-134M & 61.4 & 56.4 \\
   \modelname & \datasetname-134M & 60.3 & 54.8 \\
   \bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{ \textbf{\modelname achieves competitive zero-shot image recognition.} IN and IN-v2 denote ImageNet and ImageNet-v2 accuracy, respectively. $^\dagger$ indicates our implementation. \citet{jia2021scaling} evaluated at 640$\times$640; others evaluated at 224$\times$224. \modelname shows $\pm 0.5$ and $\pm 0.9$ IN acc. (5 runs) on {\footnotesize CC-12M} and {\footnotesize\datasetname-134M}, respectively.}
\label{table:image-recognition} 
% \vspace{-0.5em}
\end{table}
%\end{wraptable}

% CC-12M
% np.std([44.05, 44.31, 44.68, 45.3])
% HQITP-134M
% np.std([59.02, 58.33, 58.10, 60.3])
%\modelname exhibits $\pm 0.5$ and $\pm 0.9$ accuracy on IN across 5 runs.

% ALIGN Results 8/30/2022
% Pool     IN1K ZS	VOC	COCO	ADE-20K
% Avg (baseline)    49.74	29.68	14.36	7.52
% Max   45.87	33.54	15.68	7.23


==> sections/related_old.tex <==
%\vspace{-0.3cm}
\section{Related Work}

\input{sections/latex-figures/figure-arch}

{\bf Vision-language models}. Vision-language models have advanced considerably in the last decade. Early work learned correspondences between pretrained image and language embeddings to perform zero-shot image recognition \cite{frome2013devise,socher2013zero}.
Subsequent work attempted to directly predict a sentence (i.e. caption) from an associated image \cite{karpathy2015deep,vinyals2015show,kiros2014unifying,mao2014explain, desai2021virtex}.
Recent work has revisited a scaled-up version of learning correspondences between image and language features by using a cross-modal contrastive loss \cite{radford2021clip,jia2021scaling}. See \cite{pham2021combined,yu2022coca} for latest efforts in scaling up these models.

{\bf Vision-language models for grounding.}
Given the strength of vision-language models for zero-shot image recognition, several groups have extended this work to better identify the language with parts of an image. Such grounding efforts have focused on employing various heuristics to learn alignments between regions of images and words in a caption \cite{yao2022filip,cui2022democratizing} Additional work has employed language as a free form way of arbitrarily probing images in an ongoing dialogue \cite{yuan2021florence} and open vocabulary detection \cite{kamath2021mdetr}.

{\bf Semantic segmentation.}
Image segmentation is a core problem in computer vision \cite{szeliski2010computer}, and several prominent benchmarks exist for measuring success of models on a prescribed set of labels \cite{everingham2010pascal,coco,zhou2018ade}.
These benchmarks have led to a large corpus of papers focused on developing new architectures treating image segmentation as a dense supervised learning problem (e.g. \citet{chen2017deeplab,chen2018searching}).
Annotating image segmentations for supervised learning is expensive. This expense has motivated learning segmentations from weakly labeled data (e.g. \citet{pinheiro2015image}) with the goal of predicting segmentations for objects never previously observed. Several works have extended this to pursue zero-shot settings with the goal of open vocabulary segmentation. \citet{ghiasi2022open} leveraged language embeddings to segment images of unobserved visual concepts. \citet{li2022language} employed language to ground image segmentations. Finally, \citet{zabari2021semantic} employed interpretability on CLIP models to generate pseudo-labels to supervise a segmentation model.

{\bf Perceptual grouping for bottom-up recognition}.
%\todo{Revise and Expand.}
The topic of perceptual grouping has a long, rich history in human visual perception \cite{wertheimer1923} and computer vision  \cite{malik2001visual}. The central premise behind perceptual grouping is to learn representations of visual imagery that identify the affinity between visually similar objects. Perceptual grouping has been offered and explored as a method for building systems that are able to generalize to new visual domains \cite{qi2021open,malik2016three}. It is this latter goal that most closely inspires this work.

Early efforts to achieve these goals led to a series of methods in computer vision to generate groups of pixels based on known spatially-local affinities \cite{comaniciu1997robust,shi2000normalized,ren2003learning}. Subsequently, modern incarnations have led to region proposal networks for object detection \cite{uijlings2013selective} to advances in semantic segmentation \cite{arbelaez2012semantic}. Recent methods employ self-supervision to learn such grouping  \cite{cho2021picie,hamilton2022unsupervised}.
Most close to our work, GroupViT provides a custom architecture trained on vision and text pairs learning perceptual grouping by optimizing a discretized attention mask \cite{xu2022groupvit}.  



%generate segmentation and object proposals using contour detection with multi-scale information \cite{arbelaez2010contour}

{\bf Learning robust visual representations}. Assessing learned visual representations has been the subject of intense investigation. Most of the field has started this endeavor with the supposition that ImageNet accuracy provides a reasonable proxy \cite{girshick2014rcnn,kornblith2019better}. However, recent work has highlighted notable deficiencies in such learned representations \cite{geirhos2021partial,recht2019imagenet,koh2021wilds} including a sensitivity to low level textures, failures in the presence of domain shifts, and a tendency for models to rely on spurious correlations.
These failures inspired a large literature to mitigate learning spurious correlations \cite{sagawa2019distributionally,liu2021just,arjovsky2019invariant} by focusing on new optimization techniques.  Progress on this issue may address parallel issues in fairness \cite{creager2021environment}. Resulting methods have largely focused on synthetic data and arrived at algorithms for rebalancing data and shaping learned embeddings \cite{nam2020learning,liu2021just}. Nonetheless, theoretical results suggest pessimistic bounds unless additional structure informs the problem (see refs. in \citet{sagawa2019distributionally}).
%\vspace{-0.4cm}

==> sections/reproducibility.tex <==
\subsubsection*{Reproducibility Statement}
We built a codebase derived from the OpenAI CLIP source code (\texttt{https://github.com/openai}). The source code changes to accommodate our architecture were minimal, and documented in Sec. \ref{sec:methods}. We employed the pretrained \textit{Sentence T5 Base} language models from HuggingFace (\texttt{https://huggingface.co}) and a pretrained image model from \cite{caron2021emerging} and \cite{dosovitskiy2020image}. The CC-12M dataset was downloaded from \cite{changpinyo2021conceptual} and provides a publicly reproducible benchmark. \datasetname-134M can not be publicly released due to copyright issues.

==> sections/transfer-learning.tex <==
\newpage
\section{Transfer Learning of Image Representation}

Learning better generic image representations lead to gains across an array of computer vision tasks \cite{kornblith2019better,girshick2014rcnn}. Given the success of \modelname on various segmentation tasks, one natural question to ask is if the resulting image embedding may provide a useful generic image representation for other tasks \cite{radford2021clip,jia2021scaling,touvron2021training} -- particularly tasks focused on image localization \cite{huang2017speed,caron2021emerging}. We examined this hypothesis for supervised learning with object detection on the COCO dataset \cite{coco}. Briefly, we trained a DETR object detector \cite{carion2020detr} on top of the image featurization provided by \modelname, and measured the detection performance.

Tab. \ref{table:transfer-learning} reports the results in comparison to several baselines.


\begin{table}[h!]
\small
\centering
\def\arraystretch{1.2}%  1 is the default, change whatever you need
%\vspace{-0.5cm}
\begin{tabular}{c|c|cccccc}
\toprule
  & pretraining & $AP$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
   \shline
   %\;\;ALIGN $^*$ & 135M & Internal & \todo{57.5} & \todo{?} \\
   ALIGN $^\dagger$ &  \datasetname-134M & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\
   CLIP $^\dagger$ &  \datasetname-134M & \todo{?} & \todo{?} & \todo{?} & \todo{?}\\
   \modelname & \datasetname-134M & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\
   \modelname & CC-12M & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\
   \bottomrule
\end{tabular}
%\vspace{-0.3cm}
\caption{ \textbf{\modelname provides superior transfer learning for image localization.} All models evaluated at 800$\times$800 on the validation split of COCO detection \cite{coco}. $^\dagger$ indicates our implementation.}
% Superscript letter denote the result: $^a$ \citet{radford2021clip}.
\label{table:transfer-learning}  
\end{table}

==> sections/unused/grounding.tex <==


\section{Zero-shot grounding with segmentation}
\input{sections/latex-figures/table-grounding}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/IOU-Grounding-PASCAL-VOC.jpg}
\includegraphics[width=0.45\textwidth]{figures/IOU-Grounding-COCO.jpg}
\label{fig:iou-line-of-equality}
\end{center}
\vspace{-0.5cm}
\caption{{\bf Semantic segmentation and grounding across labels.} Left: PASCAL VOC 2012 across 20 classes. Right: COCO across 133 classes. Red dot indicates the mean across classes.}
% baseline mean = 50.72, 21 classes
% grounding mean = 54.01
% Processing: COCO
% baseline mean = 24.36, 133 classes
% grounding mean = 33.59
% Processing: ADE-20K
% baseline mean = 12.65, 150 classes
% grounding mean = 24.49
\end{figure}

\todo{Consider removing this section and figures/table.}

We next explored how \modelname performs on grounding. Namely, we supply the model with the set of labels we know exist in the image and ask how well the model may predict where the labeled items exist. In essence, we are asking how well the model knows {\it where} objects reside in an image given an oracle. We measure the performance of the resulting model in terms of mIoU. Table \ref{table:grounding} shows the performance of the model compared to other zero-shot methods.

We next examined how the performance of the model varies across labels. Figure \ref{fig:iou-line-of-equality} (x-axis) shows the spread grounding accuracy across the PASCAL VOC 2012 and the COCO datasets. Some labels such as {\tt chair} are quite challenging but other objects (e.g. {\tt cat}) are quite easy.

Additionally, we compare the performance of the model between the semantic segmentation and grounding task in Figure \ref{fig:iou-line-of-equality}. We see that again there is a large amount of variability in the performance on semantic segmentation, however the performance is heavily correlated with the semantic segmentation accuracy indicating that the failures of segmentation are largely due to the ability to ground certain types of objects.

==> sections/unused/methods-old.tex <==
\section{Methods}\label{sec:methods}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/Diagram-Figure.png}
\end{center}
\vspace{-0.4cm}
\caption{{\bf Diagram of architecture.} Image and caption are separately embedded into a space of depth $D$. Image embeddings are aggregated across $H\times W$ dimensions into a global embedding. A contrastive loss trains the global image embedding to be close to the caption embedding.}
\label{fig:diagram}
\vspace{-0.4cm}
\end{figure}

We first discuss the core architectures used to learn the vision and language representations of the network. We next discuss various aggregation methods explored in the paper and finally discuss pretraining and joint training. We provide additional details about the methods in the Appendix.

\subsection{Architecture}

We provide a quick overview of the vision-language architecture  (Fig. \ref{fig:diagram}). Consider a batch size $N$, spatial height $H$, spatial width $W$, and depth $D$. $X$ is a tensor that has a shape of $[N, H, W, D]$ and is the output of an image encoder. $Y$ is a tensor that is shape $[N, D]$ and is the output of a text encoder.

{\bf Language Model}. We employ a strong language model baseline derived from the transformer architecture \cite{vaswani2017attention} and implemented in T5 \cite{raffel2020exploring}. T5 models use an encoder-decoder architecture that is trained using a generative span corruption task, and have achieved state-of-the-art on a broad range of NLP tasks including GLUE~\cite{wang2018glue} and Super-Glue~\cite{wang2019superglue}. We use the encoder only and discard the decoder part. We employ the T5-base which consists of 12 transformer layers, 12 attention heads, and 768 dimensions.

{\bf Image Model}. 
We explore two architectures for image featurization, CNN-based and Vision-Transformers, although we focus the majority of work on the latter. First, we employ the EfficientNet architecture \cite{tan2019efficientnet} as a high performant CNN architecture, which has been used previously in vision-language models. The specifics of the meta-architecture were derived from considerations based on neural architecture search.
Second, we employ the Vision Transformer (ViT) architecture \cite{dosovitskiy2020image}.
%After some preliminary experiments exploring various ViT architectures across patch sizes and model sizes, we report most of our results based on ViT-B/16 model.
%This model employs patch sizes of 16$\times$16 pixels. We experiment with this model at two spatial resolutions of 224$\times$224 and 448$\times$448, resulting in 196 and 784 tokens, respectively.
%Specifically, we focus our work on ViT-B/16 and ViT-B/8 models but mostly present work with the ViT-B/16 model operating on 224$\times $224 images.
We refer the reader to \cite{dosovitskiy2020image,vaswani2017attention} for details. Briefly, ViT is largely inherited from the NLP literature and consists of a hierarchical associative memory. Each layer, termed a Transformer, is composed of a Multi-headed Self-Attention (MSA) layer followed by a 2-layer feed-forward multi-layer perceptron (MLP).
The primary parameter of ViT is the patch size $P$ specifying the $P\times P$ patch of pixels constituting a token in the architecture.

%The MSA layer is composed of $h$ self-attention modules. Each self-attention module is a weighted sum of $d$-dimensional value vectors where the normalized weight is computed based on the agreement between the queries and keys. Mathematically, the self-attention module is parameterized by matrices representing the query $Q$, key $K$, and value $V$, whose output $y={\sf softmax}\left(Q\,K^T/\sqrt{d}\right)V$ where $d$ is the dimension of the query $Q$. Each matrix is computed as a learned linear transformation of the underlying representation $x$, e.g. $Q = W_q\,x$. 

%In the NLP literature, each word is represented as a $D$-dimensional embedding vector and a sentence of $T$ tokens is represented as $T$ embedding vectors. In the ViT architecture, an image is sliced into small, square patches of a fixed $P\times P$ resolution. Each patch is akin to a single token in a NLP task. Assuming an image with a spatial resolution of $[HP, WP]$, the corresponding image contains $HW$ tokens. The network learns hierarchical interactions between the $HW$ patches to predict the class label or a semantic representation for a given image. We next discuss how to aggregate these $HW$ representations to generate the single embedding of the image.

\subsection{Aggregation}

The goal of the aggregation methods is to collapse the image embedding from a $[H, W, D]$ tensor to a $D$ dimensional vector.
Average pooling across space is an established technique for ensuring that the final embedding is independent of the image resolution \cite{szegedy2015going,long2015fully}, and has been adopted for CNN-based architectures in vision-language models \cite{jia2021scaling}.
ViT typically employs an approach from language modeling \cite{devlin2018bert}, where a {\it class token} (CLS) is prepended to the image patch tokens \cite{dosovitskiy2020image}. A class token learns an embedding that aggregates information across all patch tokens in order to predict the image label. The class token may be used to summarize the content for an entire image for ViT-based models \cite{radford2021clip,caron2021emerging}. Subsequent work in vision-language models has explored learning pooling strategies  \cite{chen2021learning,yao2022filip}, heuristically selecting a set of similar neighbors  \cite{Yun_2022_CVPR} or learning attention-based mechanisms \cite{yu2022coca}.

In this work we systematically explore how the selection of these aggregation strategies affect the ability of the model to spatially localize information. In early experiments we found that many complex strategies for aggregation yielded poor results (App. \ref{section:additional-aggregation}). We found that the simple application of maximum pooling across the spatial dimensions -- while extremely simple -- was also by far most effective (Sec. \ref{section:ablations}). We hypothesize that the success of maximum pooling may be due to the gradient updates being focused solely on a single spatial location, and not spread across all spatial dimensions.




%The goal of the aggregation methods is to collapse any representation to be $[N, D]$ (Figure \ref{fig:diagram}). Several forms of aggregation have been been explored for aggregating across spatial dimensions $[H, W]$ and word token dimension $T$ for the visual and language representations, respectively.

%For aggregating across the spatial dimensions $[H, W]$ in images, average pooling is a well established and simple technique for ensuring that the final embedding is independent of the image resolution \cite{szegedy2015going,long2015fully}, and has been adopted for CNN-based architectures in vision-language models \cite{jia2021scaling}. The recently introduced Vision Transformer (ViT) architecture employs a different approach.  As proposed in language modeling \cite{devlin2018bert}, a {\it class token} (CLS) is prepended to the image patch tokens \cite{dosovitskiy2020image}. The class token learns an embedding that aggregates information across all patch tokens in order to predict the image label. The class token may be used to summarize the content for an entire image for ViT-based models \cite{radford2021clip,caron2021emerging}.

%An additional popular method for aggregating across featurizations is to employ [CLS], a {\it class token} embedding \cite{devlin2018bert}, for an attention-based architectures. The class token is a technique for learning an embedding is that aggregates all of the content across visual tokens learned from individual patches. 

%For aggregating the image embedding, ALIGN calculates the average across all spatial locations in a CNN-based representation \cite{jia2021scaling}. CLIP proposes two methods: appending a self-attention layer on top of a CNN-based architectures, or for ViT-based architectures employing the embedding associated with the {\it class token} (CLS). The {\it class token} a token that is prepended to the image patches in a ViT which summarizes all of the information learned across all patches \cite{devlin2018bert,dosovitskiy2020image}.
%is a technique for learning an embedding is that aggregates all of the content across visual tokens learned from individual patches. 

%An additional popular method for aggregating across featurizations is to employ [CLS], a {\it class token} embedding \cite{devlin2018bert}, for an attention-based architectures. The class token is a technique for learning an embedding is that aggregates all of the content across visual tokens learned from individual patches. 

%For aggregating the language embeddings, vision-language models have employed an {\it end of sentence} (EOS) token  appended at the end of each caption \cite{radford2021clip}, or the {\it class token} (CLS) prepended to the beginning of a sentence \cite{devlin2018bert} in order to summarize the embedding for the entire sentence.

%In this work, we focus on aggregation methods for the image representation. Subsequent work in vision-language models have developed typically learned strategies for addressing aggregation across spatial dimensions. For instance, other work has explored  learning pooling strategies  \cite{chen2021learning,yao2022filip}, heuristically selecting a set of similar neighbors  \cite{Yun_2022_CVPR} or learning attention-based mechanisms \cite{yu2022coca} (see also \citet{radford2021clip}).

% In our work we explore several simple forms of aggregation method to encourage the learned representation to be more spatially localized in the image representation. We emphasize that our goal is to identify a minimal number of small changes that have maximal effect on perceptual grouping. We focus on exploring the space of pooling which require no introduced learned parameters. In particular, we examine various forms of selectively updating the image representation at only subsets of spatial locations through variations of maximum pooling. Rather than update the gradients across all spatial locations to associate with the language embedding, the goal of this method is to instead focus the model on gradient updates at only subsets of locations that maximally corresponds to the language embedding. \todo{Add more information depending on what we explore in the weeks ahead.}

\vspace{-0.2cm}
\subsection{Pretraining}

{\bf Language Model}. For better sentence representation, we initialize the T5 encoder from the pre-trained Sentence-T5 checkpoints~\cite{ni2021sentence} which adopts the original T5 models to sentence embedding models using a contrastive loss. The model is first trained on 2 billion question-answers pairs from community question-and-answer websites \citep{cer2018universal}, and is subsequently trained again using a contrastive loss on the Stanford Natural Language Inference (SNLI) dataset containing 275K examples focused on entailment questions \citep{bowman2015large,gao2021simcse}.


{\bf Image Model}. We investigate initializing the image model with several methods. First, we investigate initializing the image model using supervised learning and removing the final layer for logistic regression \cite{girshick2014rcnn,kornblith2019better}. We next investigated self-supervised methods derived from self-distillation (e.g. \cite{caron2021emerging}). We focused on this latter direction because such models demonstrated impressive performance in terms of localization.
%We focus our analysis and presentation on these latter results.
%For both pretraining methods, we employ the ImageNet dataset \citep{deng2009imagenet} with or without labels, respectively.
%\todo{Add discussion about the degree of localizaiton information in DINO. Point out self-attention on CLS token provides segmentation for DINO.}

\subsection{Joint Training}

%Consider a batch size $N$, spatial height $H$, spatial width $W$, and depth $D$. $X$ is a tensor that has a shape of $[N, H, W, D]$ and is the output of an image encoder. $Y$ is a tensor that is shape $[N, D]$ and is the output of a text encoder. 
Let $x_i$ and $y_i$ be $i$'th example in the batch for image and text embedding. A contrastive loss may be specified as the cross entropy across a batch \cite{radford2021clip,jia2021scaling}. The cross entropy is calculated between a one-hot encoding specifying the correspondence between the image and text examples, and a normalized distribution specifying the similarity between image and text embeddings.
\vspace{-0.3cm}
\begin{equation*}
\scriptsize
L = \underbrace{-\frac{1}{N}\sum_{i=1}^N\log{\frac{\exp(x_i^\top y_i / \tau)}{\sum_{j=1}^{N} \exp(x_i^\top y_j / \tau)}}}_\text{image-to-text} \,\,+\,\, \underbrace{-\frac{1}{N}\sum_{i=1}^N\log{\frac{\exp(y_i^\top x_i / \tau)}{\sum_{j=1}^{N} \exp(y_i^\top x_j / \tau)}}}_\text{text-to-image} 
\end{equation*}
The normalization for the image-to-text and text-to-image similarity is computed by summing over the potential matches (indexed by $j$) to the text and image examples within a batch, respectively. Note that $\tau$ is the temperature of the softmax for the normalization.


==> sections/unused/old-figure-jaccard.tex <==
\begin{figure}[t]

%\centering
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg}
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg}
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg}
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg}
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg}
%\includegraphics[width=0.15\textwidth]{figures/Crab_Nebula.jpg} \\
%\vspace{0.4cm}

\begin{subfigure}[valign=t]{0.03\textwidth}
    %\textbf{A.} \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ % hack!
    A. \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ % hack!
\end{subfigure}
\begin{subtable}[valign=t]{0.48\textwidth}
%\begin{minipage}{0.47\linewidth}
%\begin{subfigure}[t]{0.03\textwidth}\textbf{A}\end{subfigure}
\small
\def\arraystretch{1.2}%  1 is the default, change whatever you need
  \begin{tabular}{c|cc|c}
\toprule
  & dataset & train? & VOC \\
  %&  & vision &  \\
  %& \small{dataset} & \small{supervision} & \small{ADE20K} & \small{COCO} & \small{PASCAL VOC} \\
  \shline
%  ViT       & Random                         & -      & -           & 23.6              \\
  DeiT $^a$ & \multirow{3}{*}{\small{ImageNet}} & class & 24.6  \\
  MoCo $^b$ &  & self &  28.2 \\
  DINO $^a$ &  & self  &  45.9 \\
  \hline
  DINO $^b$ & \multirow{3}{*}{\shortstack[c]{\small{CC-12M} \\ \small{YFCC-100M}}} & self & 41.8 \\
  %DINO & \multirow{3}{*}{\small{CC-12M,YFCC}} & self & 41.8 \\
  CLIP $^b$ &  & text & 28.6 \\
  GroupViT $^b$ &   & text & 51.8   \\
  \hline
  CLIP & \small{CC-12M} & text &  37.3 \\
  CLIP & \small{\datasetname-134M} & text &  38.9 \\
  \modelname & \small{CC-12M} & text &  47.5 \\
  \modelname & \small{\datasetname-134M} & text &  \textbf{54.6} \\
  \bottomrule
  \end{tabular}
  %\end{minipage}
  \end{subtable}
  %\begin{minipage}{0.50\linewidth}
\begin{subfigure}[valign=t]{0.03\textwidth}
    B. \\ \\ \\ \\ \\ \\  % hack!
    C. \\ \\ \\ \\ % hack!
\end{subfigure}
\begin{subtable}[valign=t]{0.40\textwidth}
  \centering
  %\quad
  \begin{minipage}{\textwidth}
  \includegraphics[width=0.20\textwidth]{figures/jac_im01.jpg} \hspace{-0.4em}
  \includegraphics[width=0.20\textwidth]{figures/jac_im02.jpg} \hspace{-0.4em} 
  \includegraphics[width=0.20\textwidth]{figures/jac_im03.jpg} \hspace{-0.4em}
  \includegraphics[width=0.20\textwidth]{figures/jac_im04.jpg} \hspace{-0.4em} 
  \includegraphics[width=0.20\textwidth]{figures/jac_im05.jpg}
  \end{minipage}
  \\
  \vspace{0.3cm}
  \small
  \begin{tabular}{c|c|cc}
  \toprule
  & dataset  & ADE20K & COCO \\
  \shline
  CLIP & \small{CC-12M}  & 22.9 & 20.4 \\
  CLIP & \scriptsize{\datasetname-134M}  & 24.2 & 21.6 \\
  \modelname & \small{CC-12M}  & 28.9 & 26.0 \\
  \modelname & \scriptsize{\datasetname-134M}  & 29.5 & 27.2 \\
  \bottomrule
  \end{tabular}
  %\end{minipage}
\end{subtable}
  
  \caption{\textbf{\modelname effectively groups semantically related concepts.} (A and C) All numbers report the Jaccard Similarity, which is an instance average of the IoU between proposed and annotated segmentations independent of the object label. Superscript letter denote the result: $^a$ \citet{caron2021emerging}, $^b$ \citet{xu2022groupvit}. (B) Visualizations of perceptual grouping. Each color represent one grouping learned by the model on a given image. All models employ a ViT architecture except for GroupViT and operate with a spatial resolution between 448 and 480.}
  \label{figure:jaccard-similarity}
\end{figure}

% Previous results reported in \citet{touvron2021training,chen2021empirical,radford2021clip,caron2021emerging,xu2022groupvit}

% \def\arraystretch{1.2}%  1 is the default, change whatever you need
%   \begin{tabular}{c|cc|ccc}
%   & dataset & supervision & ADE20K & COCO & PASCAL VOC \\
%   %& \small{dataset} & \small{supervision} & \small{ADE20K} & \small{COCO} & \small{PASCAL VOC} \\
%   \hline
% %  ViT       & Random                         & -      & -           & 23.6              \\
%   DeiT & \small{ImageNet} & class  & & & 24.6  \\
%   MoCo & \small{ImageNet} & self  & & &  28.2 \\
%   DINO & \small{ImageNet} & self  & & &  45.9 \\
%   DINO & \small{CC-12M, YFCC-100M} & self & & & 41.8 \\
%   CLIP & \small{CC-12M, YFCC-100M} & text & & & 28.6 \\
%   GroupViT & \small{CC-12M, YFCC-100M} & text & & & 51.8   \\
%   \hline
%   \modelname & \small{CC-12M} & text & 71.3 & 72.7 & 62.1 \\
%   \modelname & \small{\datasetname}-135M & text & 68.8 & 74.3 & 66.7 \\
%   \end{tabular}
%   \caption{\textbf{\modelname effectively groups semantically related concepts.} \textit{Top}: Visualizations of perceptual grouping. Each color represent one grouping learned by the model on a given image. \textit{Bottom}: All numbers report the Jaccard Similarity, which is an instance average of the IoU between proposed and annotated segmentations independent of the object label. Previous results reported in \citet{touvron2021training,chen2021empirical,radford2021clip,caron2021emerging,xu2022groupvit}. All models employ a ViT architecture except for GroupViT and operate with a spatial resolution between 448 and 480. \todo{Verify me.}}
%   \label{figure:jaccard-similarity}
% \end{figure}
% DeiT \cite{touvron2021training}, MoCo \cite{chen2021empirical}, DINO \cite{caron2021emerging}, and CLIP \cite{radford2021clip}

%Ours (224 PCA)	224	14x14	6	66.55	73.01	70.33
%Ours (448 PCA)	448	28x28	6	66.74	74.25	68.75
%Ours (224 PCA)	224	14x14	8	62.54	70.66	68.33
%Ours (448 PCA)	448	28x28	8	65.12	72.85	66.85



==> sections/unused/table-ablation-init.tex <==
\begin{table}[t]%
%\scriptsize
\centering
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\begin{tabular}{c|cc|ccc}
   %& \small{DINO} & \small{T5} & & \\
   
   \multirow{2}{*}{dataset} & \multirow{2}{*}{DINO init?} & \multirow{2}{*}{T5 init?} & ImageNet & \multicolumn{2}{c}{Pascal VOC} \\
   & & & \small{accuracy} & \small{mIoU} & \small{Jaccard} \\
   %dataset & \small{DINO init?} & \small{T5 init?} & ImageNet & Pascal VOC & Jaccard \\
   \hline
   \multirow{4}{*}{CC-12M} & \cmark & \cmark & 42.3 & 50.8  & \todo{?}\\
   & & \cmark & 28.9 & 32.9  & \todo{?} \\
   & \cmark & & 34.1 & 44.3  & \todo{?}\\
   & & & 25.6 & 36.7  & \todo{?}\\
   \hline   
   \multirow{4}{*}{\datasetname-135M} & \cmark & \cmark & 59.0 & 50.1  & \todo{?}\\
   & & \cmark & 49.4 & 37.3 & \todo{?} \\
   & \cmark & & 55.2 & 46.9 & \todo{?} \\
   & & & 46.4 & 37.1 & \todo{?} \\
   \hline
\end{tabular}
\caption{ \textbf{Ablation studies across pretraining methods.} All reported numbers follow previous tables.}
\label{table:ablation-initialization}  
\end{table}


==> sections/unused/table-ablations-old.tex <==
\begin{table}[t]%
\small
\centering
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\begin{tabular}{c|c|ccc}
   \multirow{2}{*}{dataset} & \multirow{2}{*}{aggregation} & ImageNet & \multicolumn{2}{c}{Pascal VOC} \\
   & & \scriptsize{accuracy} & \scriptsize{mIoU} & \scriptsize{Jaccard} \\
   \hline
   \multirow{3}{*}{CC-12M} & Max & 42.3 & 50.8 & \todo{63.4} \\
   & Avg & 44.0 & 11.6 & \todo{53.6} \\
   & Cls & 46.0 & 4.0 & \todo{54.8} \\
   \hline   
   \multirow{3}{*}{\datasetname-135M} & Max & 59.0 & 50.1 & \todo{66.7} \\
   & Avg & 55.0 & 17.9 & \todo{55.3} \\
   & Cls & 55.0 & 4.1 & \todo{58.7} \\
\end{tabular} \\
\vspace{0.6cm}
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\begin{tabular}{c|cc|ccc}
   %& \small{DINO} & \small{T5} & & \\
   
   \multirow{2}{*}{dataset} & \multirow{2}{*}{DINO init?} & \multirow{2}{*}{T5 init?} & ImageNet & \multicolumn{2}{c}{Pascal VOC} \\
   & & & \scriptsize{accuracy} & \scriptsize{mIoU} & \scriptsize{Jaccard} \\
   %dataset & \small{DINO init?} & \small{T5 init?} & ImageNet & Pascal VOC & Jaccard \\
   \hline
   \multirow{4}{*}{CC-12M} & \cmark & \cmark & 42.3 & 50.8  & \todo{63.4}\\
   & & \cmark & 28.9 & 32.9  & \todo{63.3} \\
   & \cmark & & 34.1 & 44.3  & \todo{62.4}\\
   & & & 25.6 & 23.5  & \todo{57.5}\\
   \hline   
   \multirow{4}{*}{\datasetname-135M} & \cmark & \cmark & 59.0 & 50.1  & \todo{66.7}\\
   & & \cmark & 49.4 & 37.3 & \todo{65.5} \\
   & \cmark & & 55.2 & 46.9 & \todo{66.3} \\
   & & & 46.4 & 37.1 & \todo{65.2} \\
   %\hline
\end{tabular}

\caption{ \textbf{Ablation studies} where we show performance on zero-shot image classification (measured by accuracy), top-down segmentation (measured by mIoU) and bottom-up segmentation (measured by Jaccard similarity) \textit{Top}: Ablation across aggregation methods. All models initialized with the same pretraining features. The aggregation method varies between global maximum pooling (Max), global average pooling (Avg) and using the embedding associated with the class token (Cls). \textit{Bottom}: Ablation across used pretraining methods where we can initialized the image encoder with DINO, text encoder with T5. All models employ maximum pooling (Max).}
\label{table:ablations}  
\end{table}

